A Bidirectional DeepParticle Method for Efficiently Solving Low-dimensional Transport Map Problems

This paper aims to efficiently compute transport maps between probability distributions arising from particle representation of bio-physical problems. We develop a bidirectional DeepParticle (BDP) method to learn and generate solutions under varying physical parameters. Solutions are approximated as empirical measures of particles that adaptively align with the high-gradient regions. The core idea of the BDP method is to learn both forward and reverse mappings (between the uniform and a non-trivial target distribution) by minimizing the discrete 2-Wasserstein distance (W2) and optimizing the transition map therein by a minibatch technique. We present numerical results demonstrating the effectiveness of the BDP method for learning and generating solutions to Keller-Segel chemotaxis systems in the presence of laminar flows and Kolmogorov flows with chaotic streamlines in three space dimensions. The BDP outperforms two recent representative single-step flow matching and diffusion models (rectified flow and shortcut diffusion models) in the generative AI literature. However when the target distribution is high-dimensional (4 and above), e.g. a mixture of two Gaussians, the single-step diffusion models scale better in dimensions than BDP in terms of W2-accuracy.

==> mathSymbols.tex <==
% mathSymbols.tex
% This file compiles math symbols used throughout the thesis.
% The symbols are specifically for the thesis
% General purpose math macro should be put into mystylemath.sty instead
% 
% Author:          Mulin Cheng
% Created On:      May 25th, 2012
% Last modifed:    May 25th, 2012
%

\newcommand{\Hc}{\mathcal{H}}

\newcommand{\oL}{\mathcal{L}}
\newcommand{\oLt}{\tilde{\oL}}
\newcommand{\oLo}{\mathring{\oL}}
\newcommand{\oB}{\mathcal{B}}
\newcommand{\oQ}{\mathcal{Q}}
\newcommand{\oQt}{\tilde{\oQ}}
\newcommand{\opi}{\Pi}
\newcommand{\oA}{\mathcal{A}}

\newcommand{\lap}{\Delta}
\newcommand{\convd}{\mathfrak{D}}
\newcommand{\convdp}[3]{\convd_{\bkr{#1,#2}}#3}

\newcommand{\inp}[2]{\left\langle #1 , \, #2 \right\rangle}

\newcommand{\domd}{\mathcal{D}}
\newcommand{\domo}{\Omega}
\newcommand{\domf}{\mathcal{F}}
\newcommand{\domt}{[0,T]}
\newcommand{\spcsp}{\LL^2\bkr{\domd}}
\newcommand{\spcrd}{\LL^2\bkr{\domo}}
\newcommand{\spctm}{\LL^2\bkr{\domt}}
\newcommand{\spcal}{\LL^2\bkr{\domd \times \domo}}
\newcommand{\spcai}{\LL^2\bkr{\domo \mapto \spcsp}}

\newcommand{\vU}{\vec{U}}
\newcommand{\vUt}{\tilde{\vU}}
\newcommand{\vY}{\vec{Y}}
\newcommand{\vYt}{\tilde{\vY}}
\newcommand{\vQ}{\vec{Q}}

\newcommand{\vV}{\vec{V}}
\newcommand{\vZ}{\vec{Z}}
\newcommand{\vto}{\mathring{v}}
\newcommand{\vVto}{\mathring{\vV}}
\newcommand{\Zto}{\mathring{Z}}
\newcommand{\vZto}{\mathring{\vZ}}

\newcommand{\vz}{\vec{z}}

\newcommand{\vF}{\vec{F}}
\newcommand{\vK}{\vec{K}}
\newcommand{\vW}{\vec{W}}

\newcommand{\mLa}{\mat{\Lambda}}
\newcommand{\mC}{\mat{C}}
\newcommand{\mCt}{\tilde{\mC}}
\newcommand{\mD}{\mat{D}}
\newcommand{\mDt}{\tilde{\mD}}
\newcommand{\mR}{\mat{R}}
\newcommand{\mW}{\mat{W}}
\newcommand{\mI}{\mat{I}}
\newcommand{\mA}{\mat{A}}
\newcommand{\mAt}{\tilde{\mA}}
\newcommand{\mAh}{\hat{\mA}}
\newcommand{\mcW}{\mathcal{W}}                
\newcommand{\mB}{\mat{B}}

\newcommand{\mG}{\mat{G}}

\newcommand{\opiu}{\opi_{\vU}}
\newcommand{\opiy}{\opi_{\vY}}

\newcommand{\hmpo}{\mathrm{H}}
\newcommand{\hmpn}{\mathbf{H}}

\newcommand{\mindex}[1]{\boldsymbol{#1}}
\newcommand{\minda}{\mindex{\alpha}}
\newcommand{\mindb}{\mindex{\beta}}
\newcommand{\mindr}{\mindex{\gamma}}
\newcommand{\minde}{\mathbf{e}}

\newcommand{\gvec}[1]{\boldsymbol{#1}}
\newcommand{\vxi}{\gvec{\xi}}
\newcommand{\veta}{\gvec{\eta}}
\newcommand{\vzeta}{\gvec{\zeta}}
\newcommand{\vchi}{\gvec{\chi}}
\newcommand{\vepsi}{\gvec{\epsilon}}
\newcommand{\vpsi}{\gvec{\psi}}
\newcommand{\vtheta}{\gvec{\theta}}

\newcommand{\mset}[1]{\mathfrak{#1}}
\newcommand{\sI}{\mset{I}}
\newcommand{\sIt}{\tilde{\sI}}
\newcommand{\sJ}{\mset{J}}

\newcommand{\spB}{B}
\newcommand{\spBt}{\tilde{B}}
\newcommand{\spBtt}{\tilde{\spBt}}
\newcommand{\spBs}{B^*}
\newcommand{\intdb}{\intd \spB}
\newcommand{\intdbt}{\intd \spBt}
\newcommand{\intdbtt}{\intd \spBtt}
\newcommand{\intdbs}{\intd \spBs}


\newcommand{\ten}[1]{\mathfrak{#1}}
\newcommand{\tT}{\ten{T}}
\newcommand{\tTU}{\tT^{\bkr{\vU}}}
\newcommand{\tTY}{\tT^{\bkr{\vY}}}
\newcommand{\tTH}{\tT^{\bkr{\hmpn}}}

\newcommand{\vmm}{\vec{m}}

\newcommand{\heav}{\mathbb{H}}

\newcommand{\spg}[1]{\mathfrak{#1}}
\newcommand{\spgk}{\spg{K}}
\newcommand{\spgg}{\spg{G}}
